Follow the money: a startup-based measure of AI exposure across occupations, industries and regions

The integration of artificial intelligence (AI) into the workplace is advancing rapidly, necessitating robust metrics to evaluate its tangible impact on the labour market. Existing measures of AI occupational exposure largely focus on AI's theoretical potential to substitute or complement human labour on the basis of technical feasibility, providing limited insight into actual adoption and offering inadequate guidance for policymakers. To address this gap, we introduce the AI Startup Exposure (AISE) index-a novel metric based on occupational descriptions from O*NET and AI applications developed by startups funded by the Y Combinator accelerator. Our findings indicate that while high-skilled professions are theoretically highly exposed according to conventional metrics, they are heterogeneously targeted by startups. Roles involving routine organizational tasks-such as data analysis and office management-display significant exposure, while occupations involving tasks that are less amenable to AI automation due to ethical or high-stakes, more than feasibility, considerations -- such as judges or surgeons -- present lower AISE scores. By focusing on venture-backed AI applications, our approach offers a nuanced perspective on how AI is reshaping the labour market. It challenges the conventional assumption that high-skilled jobs uniformly face high AI risks, highlighting instead the role of today's AI players' societal desirability-driven and market-oriented choices as critical determinants of AI exposure. Contrary to fears of widespread job displacement, our findings suggest that AI adoption will be gradual and shaped by social factors as much as by the technical feasibility of AI applications. This framework provides a dynamic, forward-looking tool for policymakers and stakeholders to monitor AI's evolving impact and navigate the changing labour landscape.

==> old_intro.tex <==
\begin{comment}
\textit{There will come a point where no job is needed}. These are the words of Elon Musk regarding the impact of artificial intelligence (AI) on the job market, as discussed in an interview with the U.K. Prime Minister Rishi Sunak \citep{henshall2023elon} in 2023. At the same time, public opinion is inclined to believe that AI will lead to a job crisis, as highlighted by a 2023 Gallup poll \citep{marken2023three}. However, there is an opposing school of thought. For instance, Davis Autor argues that the fear of AI eliminating a large number of jobs is misplaced \citep{autor2024applying}. Similarly, the UK government recently dismissed as "hugely speculative" a warning from the Institute for Public Policy Research (IPPR) predicting an AI-induced job apocalypse \citep{jung2024transformed}.

As these facts illustrate, the debate on AI's potential impact on the labour market is highly polarized. Beyond the differing views, whether pessimistic or optimistic, there is a common consensus among academics, policymakers, and practitioners that the AI wave is fundamentally different from previous technological revolutions \citep{staneva2023measuring}. AI technologies now have abilities that were once believed to be uniquely human. Topical examples include large language models (LLMs) such as OpenAI's GPT and Meta's Llama, which can mimic human performance in non-routinary tasks requiring complex reasoning \citep{felten2023occupational}. This probably makes AI \textit{the most significant general-purpose technology of our era} \citep{brynjolfsson2017artificial}.

Moreover, AI technologies vary widely across different jobs, sectors, and countries \citep{georgieff2021artificial}. Since many AI applications are still in their early stages \citep{mondolo2022composite}, it is crucial to invest in monitoring AI adoption and its labour market impacts to shape effective policies. This urgency was emphasized even by EU Commission President Ursula Von der Leyen at the G20 summit of 2023, where she called for a new global framework to mitigate societal risks and promote safe, responsible AI investments.

Despite extensive research, there is still no clear consensus on how exposure to AI will impact labour demand, i.e. whether these technologies will cause more unemployment by replacing workers or enhance workers' abilities, leading to higher productivity and new job creation. Indeed, empirical studies are struggling to provide policymakers with the robust evidence needed to design effective policies and regulations \citep{acemoglu2021harms, autor2022labor}.

The primary challenge is understanding what AI can and cannot do to assess its impact on occupations. Several attempts to design an occupational AI exposure metric have been proposed by academics from multiple disciplines, including economists, social scientists, cognitive psychologists, and computer scientists \citep{staneva2023measuring}. Many of these approaches are either task-based \citep{frey2017future, brynjolfsson2018can, eloundou2024gpts} or skill/ability-based \citep{felten2019occupational,felten2021occupational, martinez2020does, tolan2021measuring}. They examine occupations along with their corresponding tasks or required capabilities to determine whether these can be automated or matched by AI applications. In this way, the AI exposure of an occupation is quantified by the proportion of tasks within that occupation that AI can perform or the proportion of required capabilities that AI possesses. While tasks, capabilities, and occupations are defined using standard taxonomies like O*NET (the US occupational information network), the selection of AI applications (such as language modeling or image recognition) is either arbitrarily decided by researchers or based on benchmarks—tasks or sets of tasks specifically designed to evaluate AI performance. A major issue with these approaches is that they mostly depend on expert evaluations of AI capabilities in relation to occupational tasks. This reliance makes the process of gathering these evaluations less transparent, objective, and reproducible.

Another approach for selecting AI applications relies on AI patents \citep{webb2020,meindl2021exposure, sousa2023artificial}. Researchers link occupational descriptions from standard taxonomies to evaluate the applicability of patented technologies in the workplace. They employ natural language processing techniques to analyze patent texts' similarity to occupational descriptions. While these patent-based approaches use a more quantitative methodology compared to relying on subjective judgments from experts, a significant disadvantage is that patents may not cover most AI applications (AI algorithms themselves, being mathematical methods, are often not patentable).

A common issue with these indices, complicating the assessment of AI's effects on labour demand, is that they inherently measure the \textit{potential} impact of AI on occupations rather than its actual impact \citep{guarascio2023artificial,svanberg2024beyond}. Indeed, expert evaluations often emphasize AI's potential based on current advancements, and patents detail innovative intellectual efforts related to AI without addressing how these technologies can be practically deployed in the workplace.

This limitation may affect the current empirical research. For example, no strong evidence of labour substitution seems to emerge for occupations considered most exposed to AI according to existing indices \cite{barbieri2020testing,mondolo2022composite,green2023artificial,albanesi2023new}. However, as pointed out in \citep{guarascio2023artificial}, datasets with more actual AI applications are needed and must be taken into account, as different outcomes may emerge.

In this paper, we tackle this issue by developing a new occupational AI exposure index to measure the near-future actual exposure rather than the potential exposure of occupations. Using data on AI applications from funded startups, our index, which we call occupational AI Startup Exposure (\startupexposure), assigns an exposure score to each occupation by employing a state-of-the-art open-weight LLM to connect the descriptions of the AI applications developed by startups to job descriptions. Differently from the existing indices, \startupexposure 
effectively maps concrete future market directions, as the startups considered are all supported by venture capital investments. These investments likely reflect the \textit{latent demand} for AI adoption, i.e., the current societal interest in integrating AI into an occupation.
Moreover, using startup data is particularly relevant regarding the claim in \citep{guarascio2023artificial} mentioned above. Unlike the abstract nature of AI capabilities found in patent or benchmark datasets, AI startups are funded because they offer tangible solutions to specific problems in the execution of tasks, which often are the building blocks of occupations. 

Furthermore, the methodology used to construct the \startupexposure 
ensures full reproducibility, as we employ an open-weight LLM that can be freely and locally executed. Also, the \startupexposure remains up-to-date, as it can be easily refreshed with the status startup dataset (see the methods for more details), which is updated daily. This aligns with the urgent goals mentioned above, enabling the tracking of investments in AI applications for supporting the development of AI policy frameworks.

With the latest update of the \startupexposure (June 2024), the main empirical findings presented in this paper are as follows. We have computed a new ranking of occupations based on their exposure to AI. When compared with an existing index in the literature, specifically the AI Occupational Exposure (AIOE) index by \citep{felten2021occupational}, which measures the potential impact of AI rather than its actual impact, interesting patterns emerge. First, our findings suggest that many potentially exposed occupations are not targeted by AI startup applications. From this, we find that, given the same level of potential exposure, occupations requiring higher levels of education, experience, and a higher skill profile are actually less exposed to near-future AI applications. This contradicts mainstream results in the literature obtained with existing exposure indices, which suggest that exposure is larger for high-skilled and high-education jobs \citep{tolan2020, eloundou2024gpts, staneva2023measuring, felten2021occupational}.

In other words, the results indicate which occupation will be affected by AI the most, largely depending on financial investment and trust in AI information, rather than just potential technological feasibility. Further, \startupexposure can depict the situations where there is still insufficient interest or trust to leave expert domain occupations in the hands of AI, at least in the short term.

Finally, as additional analysis, we use the \startupexposure to create a regional exposure map of the United States, which can be straightforwardly expanded to the entire world. Also, we employed the same methodology used to build the \startupexposure to create a Startup Robotic Exposure (RSE) index, connecting the descriptions of robotic startup applications to job descriptions. We show that the joint action of AI and robotics opens the way for job disruption in manufacturing occupations, making this combination of technological waves pervasive across all occupations.

The empirical results presented in this paper represent only a fraction of the potential insights form the occupational \startupexposure. We believe that through the \startupexposure  index and its variants, it is possible to significantly advance our understanding of AI's true impact on the job market and address the previously mentioned puzzles regarding AI's effect on labour demand, such as employment shifts and other critical outcomes.
% cappello iniziale
%Artificial intelligence (AI) technology presents a highly exciting yet polarizing debate, marked by both great admiration and apprehension.
%A pivotal question for society revolves around the future of jobs and how this revolution will affect inequalities and the distribution of wealth. 
%Promoters of AI argue that human labor will gain in efficiency, diminishing the economic advantages of high-paying jobs and professions requiring significant training, as their skills become more accessible.
%Conversely, detractors insist that skill substitution will be a detriment to the future availability of well-paid jobs.


%\begin{itemize}
    %\item AI labour market exposure: the context
    
    %\item existing approaches (more general, Acemoglu and others \citep{acemoglu2018artificial,acemoglu2022artificial,montobbio2023empirics}) and AI exposure indexes -- Felten's AIOE \citep{felten2021occupational}, Webb \citep{webb2019impact}, IMF Complementarity index \citep{pizzinelli2023labor}, etcetera.
    
    %\item forward looking approach mapping "latent demand" and future market directions through start-up venture capital investment versus approaches geared at describing state of the art technical feasibility of substitution through expert-based, \textit{which roles are replaced by AI is largely driven by money and trust in AI}. 
    %\item quantitative versus qualitative approaches in understanding exposure
    %\item summary of the results
%\end{itemize}


%LITERATURE REVIEW FROM CNEL REPORT


\section{Related Literature}
\label{sec:literature}

In this section we provide a summary of the state of the art in this framework on the impact of AI on the labour market. Far from being a comprehensive review, our goal here is to provide a  brief but broad overview of methodologies and results in this burgeoning branch of literature. References are handpicked for their relevance and representativeness. Given the fast growing body of research on AI and labour markets, we will continuously update this review over the project's duration as to have a comprehensive overview in the final report.

The study of artificial intelligence's impact on the labor market encompasses diverse methodologies, each offering unique insights into the evolving landscape of employment.
Research in this field can be broadly categorized into two main approaches, each with its distinct focus and methods.

%Job Vacancies
The first approach leverages data from job vacancies, primarily sourced from online recruitment platforms (job ads) to discern the evolution of demand for specific skills   \citep{Georgieff2021, Cammeraat2021, Acemoglu2022}. 
The expansion of AI-related job positions is the result of the increasing performance of AI to address human-level capabilities.
As the AI-exposed companies start to integrate AI into their operations, they concurrently decrease recruitment for non-AI roles and adjust the skill criteria for remaining job postings.
Although this narrative is discernible at the establishment level, the overall effects of AI-driven labor substitution on employment and wage progression in highly exposed occupations and industries are presently low  \citep{Acemoglu2022}.
Researchers analyze the frequency of references to AI or related technologies in job descriptions, using these references as proxies for skill demand and technological adoption in various occupations. 
This method provides valuable insights into the changing dynamics of the labor market, particularly in countries with significant online recruitment presence. 
However, it is important to note that this approach may not capture the full scope of industries affected, especially in regions with lower online job posting presence  \citep{Georgieff2021}.
Instead, analyzing the US online job vacancies, the authors  \citep{acemoglu2022artificial} found that AI exposure is associated with both a significant decline in some of the skills previously sought in posted vacancies and the emergence of new skills.

%Occupational Structure
The second approach delves into the structure of occupations to estimate the automation potential of tasks or skills constituting a job  \citep{Frey2013, Frey2017, brynjolfsson2018can, Felten2018, Acemoglu2020, Fossen2022}. 
This method offers a broader perspective by linking to official labor market statistics, aiding in understanding global, regional, and income-based metrics. 
Studies within this framework explore the effects of technological change and automation within a task-based framework, identifying routine-biased technological change as a significant factor driving workforce displacement \citep{Autor2006, VanReenen2011, Acemoglu2022}.
They remain neutral regarding whether AI acts as a complement or a substitute, offering an overview of occupational exposure to AI that reflects the current state of each occupation  \citep{felten2021}. 
Further, within this second approach, studies can be categorized into two categories based on how AI exposure is measured.

The first category considers a connection between AI Applications and Jobs where jobs are directly linked to AI applications, and each connection is assigned a score.
Researchers develop rubrics to capture possible impacts from AI technologies and apply them to occupations or occupational tasks, generating task- or occupation-specific scores. 
Recent methodologies in this field include mapping patent descriptions to worker task descriptions and employing machine learning classifiers to estimate automation potential across occupations \citep{Webb2020, Meindl2021, sytsma2023}. 
Additionally, there is growing research on the specific economic impacts of AI technologies such as Large Language Models (LLMs), assessing their relevance to the labor market \citep{Bommasani2021, Felten2023, Korinek2023, Mollick2022, Noy2023, Peng2023}.

The second category considers the connection between AI Applications and Jobs through Skills.
This category involves linking AI capabilities to occupational abilities from databases like O*NET \citep{Felten2018, Felten2023, tolan2020}. 
By connecting AI applications to skills required for specific occupations, researchers can assess the potential impact of AI on job roles and skill requirements more directly.

\subsection*{Details of more relevant papers}

\subsubsection*{AI labour market impact through online job vacancies}
\begin{itemize}
\item 
\citep{acemoglu2022artificial} combine the AI exposure metrics introduced in \citep{felten2021, Webb2020, brynjolfsson2017can} to study the relationship between exposure (calculated with the above metrics) and features of jobs vacancies. First, they found that there is a rapid takeoff in AI vacancy postings starting in 2010 and significantly accelerating around 2015–16. Then, they found that a strong association between AI exposure and changes in the types of skills demanded by establishments. With the Felten et al. and Webb measures (and, to a lesser extent, with SML), they found that AI exposure is associated with both a significant decline in some of the skills previously sought in posted vacancies and the emergence of new skills.

\item \citep{colombo2019ai} 
present a novel set of labor market intelligence tools, utilizing machine learning to analyze web-based job vacancies in Italy. The methodology enables the determination of various skill types required across different occupations, incorporating factors such as geographic region, industry sector, educational requirements, and experience level. A skill taxonomy is created and integrated into the ESCO classification system. The research focuses on quantifying the significance of both soft and hard skills, examining their detailed structures. An application of this data to the ongoing discourse on job computerization reveals a connection between soft and digital skills and the automation likelihood of certain occupations. Additionally, the study offers insights into the interplay between hard and soft skills, exploring their potential roles as complementary or substitutable in the labor market.

\item By adopting a task-based perspective,\citep{acemoglu2020wrong} examine the impact of artificial intelligence on employment in AI-adopting, rather than producing, establishments and detect no human-AI task complementarity. While they do not find significant employment effects at the industry-level, they find evidence of a rapid growth in AI vacancies since 2010. Moreover, they document a strong association between AI exposure and changes in demand for skills, with AI-adopters reducing hiring in non-AI positions while simultaneously replacing older skills with new skills and modifying their task structure when substituting task previously performed by human labour.

\item To our knowledge, \citep{copestake2021AI} is among the few studies that build on \citep{acemoglu2020wrong}
to explore AI adoption using vacancy data in an emerging economy, in particular by looking at the impact of AI on hiring and wages in Indian service sector firms. Their findings suggest a rise in the demand and a wage premium for machine learning skills –– used as a proxy for AI adoption –– in professional services, however this is driven by the country's largest firms and in few high-tech areas -- Bangalore, Mumbai, Hyderabad, Pune, Chennai and Delhi. This growth in AI skills leads to a subsequent decline in total and non-AI hiring growth, with a net labour displacement effect across firms, and reduced wage offers for non-AI new hires. 

\item  \citep{alekseeva2021demand}  look at the changing demand for skills by focusing on AI skills in the overall economy and across all industry sectors and occupation groups in the US. Among different sectoral patterns, their findings suggest that large firms with high R\&D investments are more likely to demand for AI skills, for which employees receive a significant wage premium. AI adoption benefits highly-qualified professionals, whereas it leads to a substitution of customer service activities. More in detail, to track the diffusion of AI, the authors use data from the online job postings database provided by Burning Glass Technologies, a job-market analytics company. These data contain nearly the universe of job vacancies posted online by firms in the US giving detailed information on vacancies that request AI skills. In particular, they show that demand for AI skills, measured as the number of posted vacancies as a share of all online job vacancies, has been rapidly increasing over the analysed time period, and the growth has accelerated since 2015. Between 2010 and 2019, the absolute number of job postings looking for AI skills grew by a factor of ten in absolute numbers and by a factor of four as a proportion of total job postings. This trend lies in marked contrast with that for other computer-related skills. For instance, the demand for other computer skills, while much larger, was remarkably stable over time as a proportion of all vacancies and only grew with the general hiring growth in a good economy. Also, the demand for AI skills has exploded across all industry sectors and occupations. Predictably, the demand is highest in the IT industry and computer occupations but is not limited to them. AI adoption benefits highly-qualified professionals, especially in professional services and finance, whereas it leads to a substitution of customer service activities. Even administrative services, manufacturing, and agriculture showed significant growth in the relative demand for AI skills. Finally, they also found finds that firms with a higher proportion of AI vacancies tend to also pay higher wages to non-AI employees. This complements the findings in \citep{acemoglu2020ai} that firms demanding AI skills change the composition of occupations within the firms by hiring less for jobs at risk of replacement by AI.

%\textcolor{blue}{Related works (that study the AI and technology demand by analyzing job vacancies)} \cite{alderucci2020quantifying, arendt2023skills, hershbein2018recessions}

\end{itemize}

\subsubsection*{AI exposure metrics by connecting jobs to AI applications through skills}
\begin{itemize}
    \item  \citep{felten2021} define their measure of AI exposure  as follows. First they connect the ONET abilities (52 abilities) with 10 standard AI applications (such as "Image recognition"). This connection is survey-based, and each connection is associated with an "intensity". The exposure $A_i$ of the ability $i$ is the sum of all these intensity over all the 10 AI applications. They found that larger proportions of high-skill occupations such as professionals and managers are the most exposed to AI due to their high concentration of cognitive-based tasks. 

\textbf{Related works (that use the Felten's measure to study the relationship between AI exposure and economic development)} \citep{hatzius2023potentially, felten2023will, felten2023occupational, felten2019occupational}

\item \citep{pizzinelli2023}  modify the standard AI exposure measure of Felten et al. (the AIOE), to take into account the "complementarity" or "substitutability" of AI technology for a job. In particular, they introduce in the AIOE measure a factor $\theta_i$ for job $i$ that reduces the "exposure" (intended in its negative meaning): the higher the probability that the AI for that job is used in a "complementary way" the lower the $\theta_i$ and the lower the exposure. The term $\theta$ for each job is hand-picked by experts based on certain criteria (for example, if a job requires high training then the authors assume that it is more probable that the AI will be complementary for that job). They studied this modified AIOE in different countries (where the exposure for each country is simply the sum of the exposure for each job weighted by the number of workers for that job in that country). They found that advanced economy countries face higher exposure than emerging economies countries due to a higher employment share in professional and managerial occupations. Also, within countries, common patterns emerge both for advanced and emerging economies: Women and highly educated workers face greater occupational exposure to AI, at both high and low complementarity. Workers with higher salaries are more likely to be in occupations with high exposure but also high potential complementarity.

\textbf{Related works (that distinguish between substitute and complementary technology)} \citep{acemoglu2019automation, gmyrek2023generative, autor2022new, milanez2023impact}

\item  \citep{tolan2020} build an AI exposure metrics  connecting jobs to skills (by ONET) and skills to AI benchmark. An AI benchmark is, for example, "Chess" or "Go". The connection with the skills is based on a survey (for example, they ask "is memory important for playing chess?"), and the "intensity" between a skill and an AI benchmark is given by the intensity of research on that AI benchmark measured as the number of publications (papers, posts, blogs ecc) on that AI benchmark. Given this tripartite network, they match AI skills to jobs and assume that the higher the AI research intensity associated with the skills required for a job, the higher the AI exposure of that job. With this, they built a ranking of occupations with respect to AI impact. Moreover, they find that some jobs that were traditionally less affected by previous waves of automation may now be subject to relatively higher AI impact.

\textbf{Related works (that use AI benchmarks)} \citep{felten2018method, martinez2018accounting}

\end{itemize}



\subsubsection*{AI exposure metrics by connecting jobs to AI application directly through text similarity}
\begin{itemize}

\item \citep{webb2020}, similarly to the previous paper, use patent-task matching to identify occupations exposed to AI, broadly defined, and found that higher-wage occupations were more exposed. Their matching is not made by NLP, but simply by "words overlap" between the job description and the AI patents descriptions.

\item \citep{gmyrek2023generative} propose an AI exposure metric  computed as follows. They ask GPT4 (with a simple prompt) "Give me a score of how much chatGPT can be useful for this task". So actually their AI exposure is a "GPT" exposure metric. Once they have a score for each task, and knowing that each job is composed of many tasks, they focus on two principal parameters of the task score distribution: (i) the mean score for a given occupation, and (ii) its standard deviation (SD). Jobs with a high mean score and a low standard deviation fall into the category of high substitutability potential, as the majority of the occupation’s tasks have high exposure scores. Jobs with a high complementarity potential are at the other extreme as they have a low occupation-level mean score, but a high standard deviation of the task scores.  They found that the potential employment effects, whether complementing or substituting, vary widely across country income groups, due to different occupational structures. In low-income countries, only 0.4 percent of total employment is potentially exposed to substitution effects, whereas in high-income countries the share rises to 5.5 percent. The effects are highly gendered, with more than double the share of women potentially affected by substitution. 

\textbf{Related works (that use GPT to assign a score to a matching between a job and an AI skill)} \citep{eloundou2023gpts, eisfeldt2023generative}
    
\item  \citep{sytsma2023} base their AI exposure measure they on Natural Language Processing (NLP) to identify semantic similarities between job task descriptions and AI technology patents awarded between 1976 and 2020. The more AI technology patents are associated with a job the higher its AI exposure. They use this measure to trace out exposure over the past several decades, and estimate how exposure correlated with employment growth. They found that, in contrast to earlier decades, occupations that require more education (training) and pay higher wages have become more exposed to technology patents in general. Moreover, greater exposure to NLP, speech recognition, and evolutionary computation technology patents is associated with declines in employment growth in occupations that specialize in more routine tasks.

\textbf{Related works (that use text similarity to match jobs with technology applications):} \citep{montobbio2021labour,webb2020,kogan2022technology, carbonero2023impact}.
\end{itemize}


\subsubsection*{AI exposure metrics via expert judgement}
\begin{itemize}
\item \citep{brynjolfsson2018can} use the O*NET content model for 964 occupations in the US economy joined to 18,156 specific tasks at the occupation level, which are further mapped to 2,069 direct work activities (DWAs) shared across occupations. They score each DWA for its Suitability for ML using a slightly extended version of the task evaluation rubric in \citep{brynjolfsson2017can}. The rubric has 23 distinct statements to be evaluated on a 5-point scale varying from "strongly disagree" to "strongly agree". Values of SML offer an indication of where ML might have the greatest potential to transform a job. The discussion emphasizes the significance of task-level variability in SML within occupations, noting that while most occupations have some SML tasks, full automation of jobs is unlikely.
Finally, the paper provides summary statistics on SML measures for occupations, tasks, and activities. It explores correlations between SML scores, wage percentiles, and wage bill percentiles, indicating that ML's impact may affect different parts of the labor force than earlier waves of automation.
\end{itemize}

\subsubsection*{Reviews on AI and technology impact}
\begin{itemize}
    \item \citep{graetz2022technology} summarize some articles in the field of technology impact on the labor market and offers some lessons for policy and future research. The articles cover central issues such as how technology changes the nature of labor demand, the impact of technology on individual workers, the role of policy, as well as emerging phenomena such as Artificial Intelligence and the Gig-economy.
    \item \citep{deranty2022artificial} 
 aim at providing a detailed overview of ongoing debates within the social sciences regarding the expected effects of AI on the labor environment. Topics addressed encompass technological joblessness, management by algorithms, the gig economy, and the political dynamics surrounding AI employment. It outlines key disciplinary and methodological views on how AI influences employment, along with the challenges encountered in forecasting these impacts. It underscores two critical factors shaping the evolution and implementation of AI in the economic sphere: the drives of capitalism and the influence of nationalist tendencies.

 \item \citep{frank2019toward} address the challenges and impacts of AI and automation technologies on labor markets, particularly in the context of increasing economic inequality and the potential for widespread technological unemployment. The paper discusses key obstacles that researchers face in assessing the effects of AI and automation on the future of work. These challenges include a lack of high-quality data on the evolving nature of occupations, the absence of empirically grounded models for micro-level processes like skill substitution and human-machine complementarity, and a limited understanding of how cognitive technologies interact with broader economic and institutional dynamics, such as urban migration and international trade policy.
\end{itemize}


In conclusion, the study of AI's impact on the labor market encompasses a range of methodologies, each offering valuable insights into the changing dynamics of employment. 
From analyzing job vacancies to exploring the structure of occupations and measuring AI exposure through direct or skills-based connections, researchers continue to unravel the complex interplay between technology and workforce dynamics. 
As AI continues to evolve, adopting a multidisciplinary approach that integrates diverse methodologies will be crucial in understanding its implications for the future of work.
\end{comment}


